Locality and Singularity for Store-Atomic Memory Models

Robustness is a correctness notion for concurrent programs running under relaxed consistency models. The task is to check that the relaxed behavior coincides (up to traces) with sequential consistency (SC). Although computationally simple on paper (robustness has been shown to be PSPACE-complete for TSO, PGAS, and Power), building a practical robustness checker remains a challenge. The problem is that the various relaxations lead to a dramatic number of computations, only few of which violate robustness. In the present paper, we set out to reduce the search space for robustness checkers. We focus on store-atomic consistency models and establish two completeness results. The first result, called locality, states that a non-robust program always contains a violating computation where only one thread delays commands. The second result, called singularity, is even stronger but restricted to programs without lightweight fences. It states that there is a violating computation where a single store is delayed. As an application of the results, we derive a linear-size source-to-source translation of robustness to SC-reachability. It applies to general programs, regardless of the data domain and potentially with an unbounded number of threads and with unbounded buffers. We have implemented the translation and verified, for the first time, PGAS algorithms in a fully automated fashion. For TSO, our analysis outperforms existing tools.

==> content/illustration2.tex <==
\sschweizer{
An example that is robust under TSO but not under PSO is message passing. A thread, called writer, updates some data and then sets a flag that the update is done. Another thread, called reader, checks that the flag is set and then reads the data. At this point, the data should be updated in memory. This pattern is useful when the data to write cannot be updated atomically. We can write the program as follows:
}
\begin{alltt}\sschweizer{
\theprogram{MessagePassing}{
\thethread{\athread_1}{}{l_0}{
\thetransition{l_0}{l_1}{\thestore{data1}{1}}
\thetransition{l_1}{l_2}{\thestore{data2}{1}}
\thetransition{l_2}{l_3}{\thefence{data1,data2}}
\thetransition{l_3}{l_4}{\thestore{flag}{1}}
}
\thethread{\athread_2}{r}{l_0'}{
\thetransition{l_0'}{l_1'}{\theload{r}{flag}}
\thetransition{l_1'}{l_2'}{\thecondition{r = 1}}
\thetransition{l_2'}{l_3'}{\theload{r}{data1}}
}
}
}\end{alltt}

\sschweizer{
This version is robust. Without the fence command, there would be a violation of robustness where the store to one of the data addresses gets delayed past the store of the flag. The fence ensures that all data is updated in memory when the flag is set.
}


\subsection{Program for that Signularity does not hold}
\begin{alltt}\sschweizer{
\theprogram{NonSingularity}{
\thethread{\athread_1}{r_1}{l_0}{
\thetransition{l_0}{l_1}{\thestore{\xaddr}{1}}
\thetransition{l_1}{l_2}{\thefence{\xaddr}}
\thetransition{l_2}{l_3}{\thestore{\xaddr'}{1}}
\thetransition{l_3}{l_4}{\theload{r_1}{\yaddr}}
}
\thethread{\athread_2}{r_2}{l_0'}{
\thetransition{l_0'}{l_1'}{\thestore{\yaddr}{1}}
\thetransition{l_1'}{l_2'}{\thefence{\yaddr}}
\thetransition{l_2'}{l_3'}{\thestore{\yaddr'}{1}}
\thetransition{l_3'}{l_4'}{\theload{r_2}{\xaddr}}
}
}
}\end{alltt}

\sschweizer{
In a minimal violation, either the store of $\xaddr$ or the store of $\yaddr$ will be delayed over the load such that both loads can read the initial value $0$ like in the normal Dekker example presented above. The fence forces the delayed store to enter the all-address-buffer immediately before the second store of that thread can be executed. From this point, the second store cannot be executed directly and has to be delayed together with the first sore. \todo{Hint: We cannot do a non-singularity example with message passing. It is just not possible because the delayed store has to be fenced such that later stores will be delayed together with the first one and then also the store of the flag will be delayed which makes the program robust.}
}

==> content/minimal.tex <==
\relax 
\@setckpt{content/minimal\protect \unhbox \voidb@x \kern .06em\vbox {\hrule width.6emdepth.4exheight-.34ex}\kern .06emviolations.tex}{
\setcounter{page}{12}
\setcounter{equation}{0}
\setcounter{enumi}{0}
\setcounter{enumii}{0}
\setcounter{enumiii}{0}
\setcounter{enumiv}{0}
\setcounter{footnote}{0}
\setcounter{mpfootnote}{0}
\setcounter{part}{0}
\setcounter{section}{0}
\setcounter{subsection}{0}
\setcounter{subsubsection}{0}
\setcounter{paragraph}{0}
\setcounter{subparagraph}{0}
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{chapter}{3}
\setcounter{@inst}{1}
\setcounter{@auth}{1}
\setcounter{auco}{1}
\setcounter{theorem}{0}
\setcounter{case}{0}
\setcounter{conjecture}{0}
\setcounter{corollary}{0}
\setcounter{definition}{0}
\setcounter{example}{0}
\setcounter{exercise}{0}
\setcounter{lemma}{0}
\setcounter{note}{0}
\setcounter{problem}{0}
\setcounter{property}{0}
\setcounter{proposition}{0}
\setcounter{question}{0}
\setcounter{solution}{0}
\setcounter{remark}{0}
\setcounter{parentequation}{0}
\setcounter{float@type}{4}
\setcounter{@todonotes@numberoftodonotes}{0}
}


==> content/syntax.tex <==
\relax 
\@setckpt{content/syntax\protect \unhbox \voidb@x \kern .06em\vbox {\hrule width.6emdepth.4exheight-.34ex}\kern .06emsemantics.tex}{
\setcounter{page}{11}
\setcounter{equation}{0}
\setcounter{enumi}{0}
\setcounter{enumii}{0}
\setcounter{enumiii}{0}
\setcounter{enumiv}{0}
\setcounter{footnote}{0}
\setcounter{mpfootnote}{0}
\setcounter{part}{0}
\setcounter{section}{0}
\setcounter{subsection}{0}
\setcounter{subsubsection}{0}
\setcounter{paragraph}{0}
\setcounter{subparagraph}{0}
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{chapter}{3}
\setcounter{@inst}{1}
\setcounter{@auth}{1}
\setcounter{auco}{1}
\setcounter{theorem}{0}
\setcounter{case}{0}
\setcounter{conjecture}{0}
\setcounter{corollary}{0}
\setcounter{definition}{0}
\setcounter{example}{0}
\setcounter{exercise}{0}
\setcounter{lemma}{0}
\setcounter{note}{0}
\setcounter{problem}{0}
\setcounter{property}{0}
\setcounter{proposition}{0}
\setcounter{question}{0}
\setcounter{solution}{0}
\setcounter{remark}{0}
\setcounter{parentequation}{0}
\setcounter{float@type}{4}
\setcounter{@todonotes@numberoftodonotes}{0}
}

